CT-DQN: Control-Tutored Deep Reinforcement Learning

One of the major challenges in Deep Reinforcement Learning for control is the need for extensive training to learn the policy. Motivated by this, we present the design of the Control-Tutored Deep Q-Networks (CT-DQN) algorithm, a Deep Reinforcement Learning algorithm that leverages a control tutor, i.e., an exogenous control law, to reduce learning time. The tutor can be designed using an approximate model of the system, without any assumption about the knowledge of the system's dynamics. There is no expectation that it will be able to achieve the control objective if used stand-alone. During learning, the tutor occasionally suggests an action, thus partially guiding exploration. We validate our approach on three scenarios from OpenAI Gym: the inverted pendulum, lunar lander, and car racing. We demonstrate that CT-DQN is able to achieve better or equivalent data efficiency with respect to the classic function approximation solutions.

==> figures/Block_Schema.tex <==
\begin{figure}[htbp]
\vspace{0.3cm}
\hspace*{1em}
\centering
\begin{tikzpicture}[auto, node distance=1.8cm]
    \node [input, name=input] {};
    \node [block, right of=input] (system) {System};
    % \node [block, below of=system, right of=system, xshift=1cm] (RF) {Reward Function};
    \node [block, below of=system, xshift=-3cm , yshift=-2cm, text width=2.3cm] (RL) {Reinforcement Learning};
    \node [block, below of=RL] (CT) {Control Tutor};
    % \node [block, below of=system, left of=system, xshift=-2cm] (policyQ) {\large $\pi^R$};
    % \node [block, below of=system, left of=system, xshift=-4.4cm] (policyT) {\large $\pi^C$};
    % \node [block, below of=policyT, yshift=-0.4cm] (CL) {Control Law};

    %\draw [->] (system.est) -| node [pos=0.25] [name=S] {$x_{k+1},x_{k}$} (RL);
    \draw [-] (system) --  ++(1.4cm,0) coordinate(S1) {};
    \draw [->] (S1) -- node [pos=0.3] [name=A1] [above] {$x_{k}$} ++(0.5cm,0) coordinate(S2) {};
    \draw [-] (S1) |-  ++(0,-4.05cm) coordinate(S2) {};
    \draw [->] (S2) |-  ++(-3.11cm,0) coordinate(S3);
    \draw [->] (S2) |-  (CT);
    % \draw [->] (RF) |-  node [pos=0.1] {$r_{k+1}$} (LU);
    % \draw [->] (S1) |- (Q);
    % \draw [->] (Q) -| (policyQ);
    \draw [<-] (system.west) -- ++(-0.6cm,0) coordinate(p1){};
    \draw [-o] (p1) -- node [pos=0.3] [name=A] [above] {$u_{k}$} ++(-1.1cm,0) coordinate(p2){};
    \draw [-] (p1) |- ++(0,-3.6cm) coordinate(p3);
    \draw [->] (p3) |-  ++(-0.16cm,0) coordinate(p4);
    % \draw [-] (p1) -- ++(0,-0.5cm) coordinate(p2){};
    % \draw [->] (A) |- (RF);
    % \draw [->] (S1) |- (LU);
    % \draw [->] (A) |- (LU);
    % \draw [->] (LU) -- node [pos=0.5] [name=temp] [right] {} (Q);
    % \draw [->] (temp) -| (policyQ);
    % \draw [->] (S1) |- ([xshift=-0.3cm,yshift=-0.27cm]LU.south west) -| (CL);
    % \draw [->] (CL) -- node [pos=0.5] [name=v] [right] {{$v_{k}$}} (policyT);
    \draw [-] (RL) -- node [pos=0.5] [name=A1] [above] {$\pi^{\R{rl}}$} ++ (-2.5cm,0) coordinate(pq1){};
    \draw [-] (pq1) -- ++(0,3.5cm) coordinate(pq2){};
    \draw [-o] (pq2) -- ++(2.2cm,0) coordinate(pq3){};
    \draw [->] (RL.north) -- node [pos=0.5] [name=A2] {$\zeta_k$} ++ (0,2.6cm) coordinate(pq4){};
    
    \draw [-] (CT) -- node [pos=0.3] [name=A3] [above] {$\pi^{\R{c}}$} ++(-3.5cm,0) coordinate(pt1){};
    \draw [-] (pt1) -- ++(0,6cm) coordinate(pt2){};
    \draw [-o] (pt2) -- ++(3.2cm,0) coordinate(pt3){};

    \draw [-] (p2) -- (pq3);
    \draw[<-] ($(pt3)+(0.5cm,0.1cm)$) to [bend right]($(pq3)+(0.5cm,-0.1cm)$);
    % \draw[->]  (pq1)  to [out=-150,in=-30] (pt1);
     
\end{tikzpicture}
\caption{Schematic of the Control-Tutored Reinforcement Learning (CTRL) algorithm.}
%At each time instant $k$, the control action $u_k$ is selected by choosing either the control action suggested by the control-tutor policy $\pi^C$ or the one suggested by the RL policy $\pi^R$.} %The choice is made in accordance to a boolean variable, $\zeta$, that will be formally defined in Section \ref{sec:CTQL}.} 
\label{fig:CTQL}
\vspace{-0.5cm}
\end{figure}
